Enabling Self-aware Smart Buildings by Augmented Reality

Conventional HVAC control systems are usually incognizant of the physical structures and materials of buildings. These systems merely follow pre-set HVAC control logic based on abstract building thermal response models, which are rough approximations to true physical models, ignoring dynamic spatial variations in built environments. To enable more accurate and responsive HVAC control, this paper introduces the notion of "self-aware" smart buildings, such that buildings are able to explicitly construct physical models of themselves (e.g., incorporating building structures and materials, and thermal flow dynamics). The question is how to enable self-aware buildings that automatically acquire dynamic knowledge of themselves. This paper presents a novel approach using "augmented reality". The extensive user-environment interactions in augmented reality not only can provide intuitive user interfaces for building systems, but also can capture the physical structures and possibly materials of buildings accurately to enable real-time building simulation and control. This paper presents a building system prototype incorporating augmented reality, and discusses its applications.

==> related.tex <==
\section{Related Work}
Researchers are beginning to explore the use of augmented reality for building navigation, management, and control. The authors in \cite{diakite2016first} present opportunities and challenges involved in the use of 3D information of the indoor building environment for the purpose of indoor navigation. A method for 3D reconstruction of indoor and outdoor environments is proposed in \cite{schops20153d}. They perform several filtering steps on monochrome fisheye images to resconstruct scenes directly on a mobile device. A history of augmented reality technology, its challenges, and applications can be found in \cite{ar_review}.
\textbf{TODO: add more reviews here}

